A Bosonic Model of Quantum Holography

We analyze a model of qubits which we argue has an emergent quantum gravitational description similar to the fermionic Sachdev-Ye-Kitaev (SYK) model. The model we consider is known as the quantum $q$-spin model because it features $q$-local interactions between qubits. It was previously studied as a model of a quantum spin glass, and while we find that the model is glassy for $q=2$, $q=3$, and likely $q=4$, we also find evidence for previously unexpected SYK-like behavior for the quenched free energy down to the lowest temperatures for $q \geq 5$. This SYK-like physics includes power-law correlation functions and an extensive low temperature entropy, so we refer to the model as Spin SYK. The model is generic in that it includes all possible $q$-body couplings, lacks most symmetries, and has no spatial structure, so our results can be construed as establishing a certain ubiquity of quantum holography in systems dominated by many-body interactions. Furthermore, we discuss a generalized family of models which includes Spin SYK and which provably exhibit SYK-like physics in the solvable limit of large local Hilbert space dimension. We also comment on implications of a bosonic system with SYK-like properties for the study of holography, Hamiltonian complexity, and related topics.

==> old_files/leftovers.tex <==
\section{Field theory model}

This appendix reviews a standard field theory model of the long-range fixed point discussed in \bgs{blah}. It consists of a $K$-component field with a long-range kinetic term. As argued in the main text, the measure terms not important for the existence of the power-law solution, so we lump them into a generic UV cutoff. The \name{} model corresponds to $K=3$. There is no fully controlled way to access the relevant fixed point when $K=3$, so we discuss the large $K$ solution as an approximate guide. Crucially, the existence of the fixed point and the non-renormalization of the anomalous dimension do not depend on the large $K$ limit. \bgs{cite}

The action is
\begin{equation}
    I = - \frac{1}{2} \int d\tau d\tau' \frac{\phi(\tau) \phi(\tau')}{|\tau-\tau'|^{1+s}} + \int d\tau \frac{\lambda}{2} \left( \phi(\tau) \phi(\tau) - K r^2 \right).
\end{equation}
The kinetic term is determined by $\Sigma$, so this action arises from a power-law ansatz, $\Sigma(\tau_1,\tau_2) \sim |\tau-\tau'|^{-(1+s)}$. $\lambda$ is a fluctuating field which enforces the spherical constraint,
\begin{equation}
    \phi^2 = K r^2,
\end{equation}
thus making this a ``non-linear sigma model''. As discussed below, we restrict to $s \in (0,1)$. The parameter $r$ sets the radius of the sphere and plays the role of $\Sigma_0$ from the main text. We define the quadratic term as the Fourier transform of $C |\omega|^s$ for some constant $C$ whose precise form is unimportant.

We first discuss the solution of the field theory as a function of $r$ and $s$ without imposing the self-consistency constraint. The phase diagram is determined by solving the $\lambda$ EOM,
\begin{equation}
    \frac{\langle \phi^2 \rangle}{K} = r^2.
\end{equation}
Assuming the $O(K)$ symmetry is not broken, the $\lambda$ EOM takes the form
\begin{equation}
    \int^\Lambda \frac{d\omega}{2\pi} \frac{1}{C |\omega|^s + \lambda} = r^2,
\end{equation}
where $\Lambda$ indicates a UV cutoff at frequency $\omega = \Lambda$. For small $r$, there is always a solution obtained by making $\lambda$ large. For sufficiently large $r$, there is no solution, which indicates that the assumption of unbroken symmetry must fail.

The critical point, $r=r_c$, is determined by the condition $\lambda(r_c)=0$. This is
\begin{equation}
    \int^\Lambda \frac{d\omega}{2\pi} \frac{1}{C|\omega|^s} = \frac{\Lambda^{1-s}}{\pi (1-s) C} = r_c^2.
\end{equation}
Note that, for $s\geq 1$, the integral is IR divergent, so it isn't actually possible to have $\lambda=0$ for any finite value of $r$. This is a manifestation of the fact that the system cannot order for $s\geq 1$. For $s\leq 0$, the couplings are so long-ranged that the system always orders. Both of these cases are interesting from the field theory perspective, however, they are not relevant for the self-consistent problem we face.

In fact, the self-consistency condition forces the field theory model to sit at the critical point. For if not, then $G$ is either long-ranged (ordered phase) or decays too rapidly (disordered phase), with neither case being self-consistent with the ansatz that $\Sigma \sim \tau^{-(1+s)}$. By contrast, the correlations at the critical point are 
\begin{equation}
    \langle \phi_i(\tau) \phi_j (0) \rangle = \delta_{ij} \int^{\Lambda} \frac{d\omega}{2\pi} \frac{e^{ - i \omega \tau}}{C |\omega|^s} \sim \frac{1}{\tau^{1-s}},
\end{equation}
and these are self-consistent with couplings $\Sigma \sim \frac{1}{\tau^{1+s}}$ provided
\begin{equation}
    s = 1 - \frac{2}{q}.
\end{equation}

We close by emphasizing again that this analysis is strictly correct only in the limit of large $K$, however, the scaling of the correlations with $\tau$ is known to be exact. \bgs{more?}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% We work perturbatively in $\Sigma$, starting from the representation
%\begin{equation}
 %   G(\tau) = \frac{\int Dh \tr(\mathcal{P}( e^{\int d\tau' h_\nu(\tau') \sigma_\nu(\tau')} \sum_\mu \sigma_\mu(\tau) \sigma_\mu(0) ) )}{\int Dh \tr(\mathcal{P}( e^{\int d\tau' h_\nu(\tau') \sigma_\nu(\tau')} ) )}.
%\end{equation}
%The denominator is
%\begin{equation}
%    {\int Dh \tr(\mathcal{P}( e^{\int d\tau' h_\nu(\tau') \sigma_\nu(\tau')} ) )}=2 + 6 \int d\tau' d\tau'' \Sigma(\tau',\tau'') + \cdots,
%\end{equation}
%and the numerator is
%\begin{equation}
%\begin{split}
%    {\int Dh \tr(\mathcal{P}( e^{\int d\tau' h_\nu(\tau') \sigma_\nu(\tau')} \sum_\mu \sigma_\mu(\tau) \sigma_\mu(0) ) )}=6 + \int d\tau' d\tau'' \Sigma(\tau',\tau'') \sum_{\mu \nu }\tr( \mathcal{P}(\sigma_\nu(\tau') \sigma_\nu(\tau'') \sigma_\mu(\tau) \sigma_\mu(0)))+ \cdots=\\
%    6+   6 \int d\tau' d\tau'' \Sigma(\tau',\tau'') +    12 \int d\tau' d\tau'' \Sigma(\tau',\tau'') \text{sgn}(\tau'-\tau) \text{sgn}(\tau''-\tau).
%\end{split}
%\end{equation}
%Hence, we have 
%\begin{equation}
%    G (\tau) = 3 \left( 1 + 2\int d\tau' d\tau'' \Sigma(\tau',\tau'') [ -\frac 12 +\text{sgn}(\tau'-\tau) \text{sgn}(\tau''-\tau)] + \cdots \right).
%\end{equation}

%By taking derivatives, we find that 
%\begin{equation}
%    \partial_\tau^2 g = 2 \mathcal{J}^2 e^g
%\end{equation}
%with
%\begin{equation}
%    \mathcal{J}^2 = 4q 3^{q-1} J^2.
%\end{equation}
%The standard solution is
%\begin{equation}
%    e^g = \left[ \frac{\cos \frac{\pi v}{2}}{\cos \left[ \pi v \left(\frac{1}{2} - \frac{\tau}{\beta}\right)\right]}\right]^2
%\end{equation}
%\begin{equation}
%    \beta \mathcal{J} = \frac{\pi v}{\cos \frac{\pi v}{2}}.
%\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%

\section{(New) $q$-local Quantum Model}

This section deals with a generalization of the \name, which we called the $q$-local Quantum Model. To explain the generalization, it is useful to view \name{} model as obtained from $q$-body interactions where the contribution of each site is a generator of SU($2$) in the fundamental representation. This suggests a generalization in which we instead take generators of SU($M$) in some representation $R$. Each of the $N$ sites will then carry states to fill out the chosen representation. For example, if $R$ is the fundamental, then we are simply constructing $q$-body terms built from a complete basis of Hermitian operators on an $M$-level system. This generalization is interesting on its own terms, as a more general kind of $q$-local quantum system, and because the large $M$ limit gives additional analytical constrol.

It will be useful and interesting to consider a variety of choices for $R$. In particular, we can distinguish three natural families of models, all of which limit to SU($2$):
\begin{itemize}
    \item{[Family 1]} $R$ is the antisymmetric product of $k$ fundamentals. This case is naturally solved using \textit{fermionic spinons} at large $M$. The limit $k=1/2$, $M=2$ is the \name{} model.
    \item{[Family 2]} $R$ is the symmetric product of $k$ fundamentals. This case is naturally solved using \textit{bosonic spinons} at large $M$. The limit $k=1/2$, $M=2$ is the \name{} model.
    \item{[Family 3]} $R$ is the fundamental of SU($M$). The limit $M=2$ is the \name{} model.
\end{itemize}
We will focus primarily on Family 1, which yields SYK-like physics at large $M$ and, based on the finite size numerics, is most likely to capture the dynamics at $M=2$ for $q>3$. Family 2 is better able to access glassy states (essentially because bosons can easily condense). Family 3 is also the limit of Families 1 and 2 when $k=1/M$; we discuss it in more detail below.

For each family, the Hamiltonian is formally the same when expressed in terms of the generators, $T_{r\mu}$, which is the $1\leq \mu\leq M^2-1$th generator of SU($M$) acting on site $1\leq r \leq N$ \cite{Haber:2019sgz}. The Hamiltonian is
\begin{equation}
    H=\sum_{r_1\mu_1 \cdots r_q \mu_q} J_{r_1 \mu_1 \cdots r_q \mu_q} T_{r_1 \mu_1} \cdots T_{r_q \mu_q},
\end{equation}
with 
\begin{equation}
    \av{J_{r\mu \cdots}^2}=\frac{(q-1)! J^2}{N^{q-1}}.
\end{equation}
There are ${N\choose q} (M^2-1)^q$ terms contributing to the sum. 

By employing SU($M$) coherent states \bgs{cite}, one can write down an analogous path integral for the QQ model. We will not need the details of that path integral, so we proceed schematically here. If we add in a Lagrange multiplier
\begin{equation}
    S_{\textrm{Lagrange}}= N \int d\tau_1 d\tau_2 \Sigma(\t_1,\t_2)\left(G(\t_1,\t_2)-\frac 1N\sum_{r\mu}T_{r\mu}(\t_1)T_{r\mu}(\t_2)\right)
\end{equation}
and follow the same manipulations as in Section \ref{sec:Action}, then the action becomes 
\begin{equation}
       \int D\Sigma D G  \exp\left(N\frac{J^2 }{2 q} \int G^qd\t^2 - \frac{N}{2} \int \Sigma G d\t^2+ N\log \langle\mathcal P e^{\int \sum_\mu T_\mu h_\mu(\tau) d\t}\rangle_{\Sigma} \right),
\end{equation}
with equations of motion
\begin{equation}
    \Sigma = J^2 G^{q-1}
\end{equation}
and
\begin{equation}
    G = \big \langle \sum_\mu T_\mu(\tau_1) T_\mu(\tau_2) \big \rangle_{\Sigma}.
\end{equation} 
As with \name{}, $G$ is determined by solving a single-site problem with a magnetic field in the adjoint representation whose covariance is specified by $\Sigma$.

\subsection{Solving the Single-Site Problem}

We can solve the single-site problem in different ways depending on the family of interest. Here we consider Family 1, which corresponds to the antisymmetric product of $M/2$ fundamentals ($M$ must be even). \bgs{cite subir}

We introduce fermionic ``spinons'' $f_\alpha$ where $\alpha=1,\cdots,M$ which transform in the fundamental of SU($M$). Then the generators can then be expressed as
\begin{equation}
    S^{\alpha}_\beta= f^\dagger_\beta f^\alpha - k \delta^\alpha_\beta.
\end{equation}
With the constraint that 
\begin{equation}
    \sum_\alpha f_\alpha^\dagger f^\alpha = k M,
\end{equation}
one can verify that these generators obey the Lie algebra and transform in the antisymmetric produce of $k$ fundamentals. Note that $(S^\alpha_\beta)^\dagger = S^\beta_\alpha$, so the Hermitian generators $T_\mu$ are obtained from the real and imaginary parts of the $S$s with $\alpha \neq \beta$. 

The local Hilbert space on each site has dimension $ \binom{M}{kM}$. From the formula
\begin{equation}
    \sum_{\alpha \beta} S^\alpha_\beta S^\beta_\alpha = k(1-k)M(M+1),
\end{equation}
we find that 
\begin{equation}
    G(0) = k(1-k)M(M+1).
\end{equation}
For $M=2$, this differs from our previous convention by a factor of $1/2$.
